Surveying the onset and evolution of supermassive black holes at high-z with AXIS

The nature and origin of supermassive black holes (SMBHs) remain an open matter of debate within the scientific community. While various theoretical scenarios have been proposed, each with specific observational signatures, the lack of sufficiently sensitive X-ray observations hinders the progress of observational tests. In this white paper, we present how AXIS will contribute to solving this issue. With an angular resolution of 1.5$^{\prime\prime}$ on-axis and minimal off-axis degradation, we have designed a deep survey capable of reaching flux limits in the [0.5-2] keV range of approximately 2$\times$10$^{-18}$ \fcgs~ over an area of 0.13 deg$^2$ in approximately 7 million seconds (7 Ms). Furthermore, we have planned an intermediate depth survey covering approximately 2 deg$^2$ and reaching flux limits of about 2$\times$10$^{-17}$ \fcgs ~ in order to detect a significant number of SMBHs with X-ray luminosities (L$_X$) of approximately 10$^{42}$ \lx up to z$\sim$10. These observations will enable AXIS to detect SMBHs with masses smaller than 10$^5$ \ms, assuming Eddington-limited accretion and a typical bolometric correction for Type II AGN. AXIS will provide valuable information on the seeding and population synthesis models of SMBH, allowing for more accurate constraints on their initial mass function (IMF) and accretion history from z$\sim$0-10. To accomplish this, AXIS will leverage the unique synergy of survey telescopes such as JWST, Roman, Euclid, LSST, and the new generation of 30m class telescopes. These instruments will provide optical identification and redshift measurements, while AXIS will discover the smoking gun of nuclear activity, particularly in the case of highly obscured AGN or peculiar UV spectra as predicted and recently observed in the early Universe.

==> Definitions/journalnames.tex <==
\DeclareOption{ArXiv}{ 	    \gdef\@journal{ArXiv}	\gdef\@journalshort{ArXiv}	\gdef\@journalfull{ArXiv}	\gdef\@doiabbr{ArXiv}	}
